Ray-Based Reflectance Model for Diffraction

We present a novel method of simulating wave effects in graphics using ray--based renderers with a new function: the Wave BSDF (Bidirectional Scattering Distribution Function). Reflections from neighboring surface patches represented by local BSDFs are mutually independent. However, in many surfaces with wavelength-scale microstructures, interference and diffraction requires a joint analysis of reflected wavefronts from neighboring patches. We demonstrate a simple method to compute the BSDF for the entire microstructure, which can be used independently for each patch. This allows us to use traditional ray--based rendering pipelines to synthesize wave effects of light and sound. We exploit the Wigner Distribution Function (WDF) to create transmissive, reflective, and emissive BSDFs for various diffraction phenomena in a physically accurate way. In contrast to previous methods for computing interference, we circumvent the need to explicitly keep track of the phase of the wave by using BSDFs that include positive as well as negative coefficients. We describe and compare the theory in relation to well understood concepts in rendering and demonstrate a straightforward implementation. In conjunction with standard raytracers, such as PBRT, we demonstrate wave effects for a range of scenarios such as multi--bounce diffraction materials, holograms and reflection of high frequency surfaces.

==> concept.tex <==
% !TEX root = ./wbsdf.tex
\subsection{Concept}

%\TODO{Tom Cuypers}{Describe angles}

%\TODO{TC}{Schematic for explaining concept}

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{images/brdf.pdf}
\caption{We derive the BSDF for a sinusoidal grating and use it for rendering (a) the WDF for the microstructure, where red defines positive values and blue means negative (b) the phase function of the structure (c) the WBRDF for the structure (b) at different positions (d) Rendering using the WBRDF}
\label{fig:brdf}
\end{figure}

Rendering photo realistic images in computer graphics is often implemented by solving the rendering equation~\cite{Kajiya1986}:
\begin{linenomath}
\begin{multline}
L_{o} ( x, \theta_{o}, \lambda ) = L_{e} ( x, \theta_o, \lambda ) +\\ 
 \int_{\Omega } f_r ( x, \theta_o, \theta_i, \lambda ) L_i( x, \theta_i, \lambda ) (-\theta_i \cdot n ) \text{d} \theta_i,
 \label{eq:render_eq}
\end{multline}
\end{linenomath}
where $L_o( x, \theta_o, \lambda )$ is the total outgoing light from the point $x$ in the direction $\theta_o$ with the wavelength of $\lambda$. $L_e$ describes the light emitted at the point $x$ in the direction $\theta_{o}$, and $L_i$ denotes the incoming light at the point from a certain direction. $\Omega$ is the hemisphere of all incoming directions. The function $f_r$ represents the proportion of reflected or transmitted light for a given incoming and outgoing direction, and $f_{r}$ is often referred to as the Bidirectional Reflectance Distribution Function (BRDF) or BTDF in case of transmission. 

As eq.~\eqref{eq:render_eq} only takes the intensity of rays into account, and no phase information, interference between multiple rays cannot be described. Previous works have described how to add local diffraction and interference effects to the BRDF~\cite{Stam1999}. However, a traveling ray does not encode phase information in it and therefore is unable to interfere in a later stage.

%\TODO{SB}{Following sentence should be changed since we took the figure out.} Figure~\ref{fig:spatial_freq} illustrates the concept of the local spatial frequency, where a point light source emits an omnidirectional light wave. We plot the intersection of the surface and the incoming light wave. 


In optics, light transport as waves is often described using the Wigner Distribution Function (WDF), which is a function of position $x$ and spatial frequency $u$. Spacial frequency represents how fast phase varies over space, typically a surface normal to the propagation direction.  The phase varies in a sharp fashion and the frequency of the phase oscillation in the space domain (in this case along the $x$--axis) is the local spatial frequency. This local spatial frequency is related to the direction of rays, which is normal to the wavefront, and the wavelength as
\begin{linenomath}
\begin{equation}
u = \frac{\sin \theta }{\lambda}.
\end{equation}
\end{linenomath}

As pointed out in previous research~\cite{Zhang2009,Oh2009}, the WDF and lightfields exhibit similar representation and properties because both of them describe light in position--angle (or spatial--frequency) space:
\begin{linenomath}
\begin{equation}
 \textrm{LF}( x, \theta ) \sim \mathcal{W}\left( x, \frac{\textrm{sin}\theta}{\lambda} \right).
\end{equation}
\end{linenomath}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{images/concept.pdf}
\caption{\TODO{TC}{todo - dont really knwo what to put in this image yet}}
\label{fig:brdf}
\end{figure}

With this knowledge we represent a ray %, which is a subset of the lightfield, 
with the WDF $\mathcal{W}$ as
\begin{linenomath}
\begin{eqnarray}
L_i(  x, \theta_i, \lambda ) &\sim& \mathcal{W}_i\left( x, \frac{\sin \theta_i}{\lambda} \right),\\
L_e( x, \theta_o, \lambda ) &\sim& \mathcal{W}_e\left( x, \frac{\sin \theta_o }{\lambda} \right),\quad\text{and}\\
L_o( x, \theta_o, \lambda ) &\sim& \mathcal{W}_o\left( x, \frac{\sin \theta_o }{\lambda} \right).
\end{eqnarray}
\end{linenomath}
When light is transmitted through a mask, the WDF of the incident light is transformed due to the microstructure of the mask. If the structure is sufficiently thin, this transformation becomes angle shift--invariant; the transmitted light pattern rotates in the same fashion as the incident light rotates. This is a reasonable approximation when the lateral size of a patch is significantly larger than the thickness of the microstructure. If we assume the angle--shift invariance, then 
\begin{linenomath}
\begin{equation}
\mathcal{W}_o( x, u_o ) = T_t( x, u_o - u_i ) \mathcal{W}_i( x, u_i ),
\end{equation}
\end{linenomath}
where $W_t$ is the transmitted wavefront for an incoming wavefront $W_i$. $T_t( x, u_o - u_i )$ is solely dependent on the microstructures geometry $g(x)$ and can be calculated using the well--studied WDF:
\begin{linenomath}
\begin{multline}
T_t( x, u ) = \mathcal{W}_{t}(x,u)\\
            = \int { t\left( x + {x' \over 2} \right) t^{*}\left( x - {x' \over 2} \right) e^{-i 2 \pi x' u} \text{d}x'},\quad
            \label{eq:T_t_WDF}
\end{multline}
\end{linenomath}
where $t(x)$ is a complex function describing amplitude and phase variation of light due to the surface structure. Note that $T_{t}(x,u)$ may contain positive as well as negative real--valued coefficients. However, after integration of all incoming wavefronts, the integrated value -- \textit{intensity} -- always becomes non--negative~\cite{Bastiaans1997}.
For reflections we assume that the reflected wavefront is a mirror of the transmitted wavefront and therefore $T_r( x, -u_o - u_i ) = T_t( x, u_o - u_i )$.
This allows us to derive BSDFs with wave properties:
\begin{linenomath}
\begin{equation}
f_r( x, \theta_i, \theta_o, \lambda ) \sim \mathcal{W}_{t}\left( x, \frac{-\sin \theta_o  - \sin \theta_i}{\lambda} \right).
\label{eq:brdf_as_wdf}
\end{equation}
\end{linenomath}
Although our WBSDF may contain negative coefficients, the final intensity becomes non--negative since the WDF is assured to be positive after integration over all incoming light, and the negative coefficients allow us to model diffraction and interference conveniently.

In order to create the WBSDF, we need to know the exact microstructure of the material. This structure can be separated into an amplitude $a(x)$ and a phase component $\Phi(x)$. The amplitude defines how much of the light are reflected or absorbed. The phase component defines the phase delay between incoming and outgoing light. It can therefore be seen as a heightfield where rays have to travel a different distance and have different phases. The geometric structure is described as
\begin{linenomath}
\begin{equation}
t(x) = a(x) e^{i 2 \pi \Phi(x)},
\end{equation}
\end{linenomath}
which can directly be exploited to create the BRDF in eq~\eqref{eq:brdf_as_wdf}. We show an example in figure~\ref{fig:brdf}, where we derive a BRDF for a sinusoidal phase grating surface and use it for rendering.

\begin{figure}[t!]
     \centering
     \subfigure[Spotlight on cd]
     {
         \includegraphics[width=.225\textwidth]{images/cd-real.pdf}
     }	
     \subfigure[Rendering scene (a)]
     {
          \includegraphics[width=.225\textwidth]{images/cd-render.pdf}
     }	
     \subfigure[Light reflecting from 1 CD into another CD]     
     {
          \includegraphics[width=.225\textwidth]{images/cds-real.pdf}
     }	     
     \subfigure[Rendering scene (c)]
     {
          \includegraphics[width=.225\textwidth]{images/cds.pdf}
     }
     \caption{Some results rendered using our Wave based BRDF in PBRT using global illumination.}
     \label{fig:results}     
\end{figure}



The same principles can be used for rendering audio using raytracing, with the difference of having larger wavelengths. We can even extend this idea to improve the emision function $L_e$ by taking phase information into account. Let's assume that we know the phase difference between several emissive points, the outgoing light will not create a planar wave. This effect is especially noticeable in longer wavelength spectrum such as audio. When several speakers emit the same sound, but have a slight different time delay, we will not hear the same sound at every location. 
%This is the same as propagating a wave through a phase grating $\Phi(x)$ resulting in different phases of outgoing rays. Therefore we can write the emission function as
%\begin{linenomath}
%\begin{equation}
%L_e( x, \theta_o, \lambda ) = \mathcal{WDF}\left( x, \frac{\sin \theta_o}{\lambda} \right)
%\end{equation}
%\end{linenomath}
%edited by SB as follows
This emissive effect is equivalent to a propagating wave through a grating $t(x)$ with different amplitudes and phase delays $\psi(x)$. Thus, we can write the emission function as
\begin{linenomath}
\begin{equation}
L_e( x, \theta_o, \lambda ) = \mathcal{W}_{t}\left( x, \frac{\sin \theta_o}{\lambda}-\frac{\partial\psi(x)}{\partial x}\right).
\end{equation}
\end{linenomath}

\TODO{TC}{Why phase function inside function?}
\TODO{SB}{$\psi$ is different from $\Phi$. I realized that partial derivative of the phase is corresponding to the spatial frequency.}






%\begin{figure}[t!]
%\centering

%\subfigure[WDF of a rectangular aperture]{
%\includegraphics[width=0.3\columnwidth]{images/wdf-rec_aperture.pdf}
%}
%\subfigure[transformation of light bundle through aperture]{
%\includegraphics[width=0.3\columnwidth]{images/propagate-rec_aperture.pdf}
%}
%\subfigure[projection of light bundle]{
%\includegraphics[width=0.3\columnwidth]{images/project-rec_aperture.pdf}
%}
%\caption{(a) We show the Wigner Distribution function of a rectangular aperture (b) shows how an incoming light bundle propagates through this aperture. The intensities of the outgoing ray bundle is defined by the WDF in (a) (c) When we project the light bundle on a diffuse plane we will end up with this non-negative fraunhofer pattern.}
%\label{fig:rec_aperture_example}
%\end{figure}

%\begin{figure*}[t!]
%  \includegraphics[width=0.9\textwidth]{images/overview.pdf}


%  \caption{Left we have the WDF for a sinusoidal phase grating surface. We can create a brdf for a position $x$ by taking the column out of this function and shearing it for $\theta_{in}$ and $\theta_{out}$ for each wavelength as $\theta = \frac{\theta_{in} - \theta_{out}}{\lambda}$. We show BRDFs for 4 different positions on the surface. As presentated on the right, the reflection from different positions can  end up together and create destructive interferences by integrating over positive and negative light. The right bottom describes the reflected light in x - $\theta$ space. The values contributing to a single pixel are indicated. This integration can be done most rendering frameworks by defining the pixel size and aperture size of the virtual camera}
%  \label{fig:overview}
%\end{figure*}


%We construct a BRDF and BTDF for simulating wave phenomena based on the Wigner Distribution function, which is popular in wave optics. This function defines for a bundle of incoming light rays how they will propagate. We illustrate this with a simple example in figure~\ref{fig:WD}. Assuming the transmitting surface is infinitely thin, this function is angle-shift invariant. This means that when the bundle of incoming light rays rotates, the outgoing propagation is rotated in a similar fashion. In flatland, we can simply describe this light transformation function as:

%\begin{equation}
%I( x, \theta_{out} ) = \textrm{f}\left( x, {\theta_{out} - \theta_{in} \over \lambda} \right) I(x, \theta_{in})
%\label{eq:wdf-brdf}
%\end{equation}

%Where $\textrm{f}\left( x, {(\theta_{out} - \theta_{in}) \over \lambda} \right)$ contains positive, as well as negative valued coefficients. One property of the WDF is when we project this bundle of light onto a surface, we will always end up with non-negative intensities.

%An example of the WDF of a rectangular aperture is shown on Figure~\ref{fig:rec_aperture_example}(a). Notice that this function contains positive (red), as well as negative coefficients (blue). In this equation $\theta = {{\theta_{out} - \theta_{in}} \over {\lambda}}$, with $\lambda$ the wavelength of the propagating light.

%Even though this function is shift invariant, we obtain different patterns watching from different positions. This is due to the interference of the rays coming in from different angles as shown on Figure~\ref{fig:rec_aperture_example}(b). Here we see that at some positions on the second diffuser, there are positive and negative light rays getting together, cancelling each other out (Figure~\ref{fig:rec_aperture_example}(c)). 
